Accelerating Task-based Iterative Applications

Task-based programming models have risen in popularity as an alternative to traditional fork-join parallelism. They are better suited to write applications with irregular parallelism that can present load imbalance. However, these programming models suffer from overheads related to task creation, scheduling and dependency management, limiting performance and scalability when tasks become too small. At the same time, many HPC applications implement iterative methods or multi-step simulations that create the same directed acyclic graphs of tasks on each iteration. By giving application programmers a way to express that a specific loop is creating the same task pattern on each iteration, we can create a single task DAG once and transform it into a cyclic graph. This cyclic graph is then reused for successive iterations, minimizing task creation and dependency management overhead. This paper presents the taskiter, a new construct we propose for the OmpSs-2 and OpenMP programming models, allowing the use of directed cyclic task graphs (DCTG) to minimize runtime overheads. Moreover, we present a simple immediate successor locality-aware heuristic that minimizes task scheduling overhead by bypassing the runtime task scheduler. We evaluate the implementation of the taskiter and the immediate successor heuristic in 8 iterative benchmarks. Using small task granularities, we obtain an average speedup of 3.7x over the reference OmpSs-2 implementation and an average of 5x and 7.46x speedup over the LLVM and GCC OpenMP runtimes, respectively.

==> sections/background.tex <==
\section{Background}
\label{sec:background}

Many of the applications that scientists run on HPC clusters are iterative, which means they
perform similar operations multiple times until they converge on an approximate result.

An example of iterative applications are those that solve nonlinear or very large linear systems of equations.
We apply iterative methods in these applications because direct methods only exist for a subset of the nonlinear
equation space and are too expensive to compute for large linear systems.
One application of this class is the Conjugate Gradients method~\cite{conjugate}, used to solve positive-definite sparse linear equation systems.
This case is especially relevant for HPC because it is implemented in the HPCG benchmark~\cite{hpcg}.

Another class of iterative applications are multi-step simulations, which reproduce how a system
changes through a series of timesteps. This is the case for N-Body simulations or Full-Wave Inversion methods.

Moreover, modern machine learning algorithms are also iterative during their training phase.
Training is done by processing a small input batch, calculating a cost function, performing back-propagation, and repeating the process for many iterations.

In the last years, task-based programming models have been used to address load imbalance in parallel applications.
Additionally, they allow overlapping communication and computation phases \cite{CastilloOverlap2019, sala2020towards, tampi},
an essential optimization in distributed iterative applications.
Nevertheless, data-flow programming presents some inefficiencies in dealing with iterative patterns.
When using tasks, programmers have to balance the overhead of task creation and scheduling with the duration of each task.
More importantly, the core that creates the tasks has to do so fast enough to feed all other available cores.
When the creator thread is too slow, performance can drop dramatically.
However, there is no way for programmers to express that each iteration of a loop will always generate the same task DAG,
and hence it could be reused instead of being created multiple times.

\subsection{An Example: The Gauss-Seidel Method}
Let us illustrate this problem with a specific example, without loss of generality.
The Gauss-Seidel method is an iterative method used to solve linear equation systems.
It is guaranteed to converge when applied to strictly diagonally dominant matrices, making it suitable
to solve Partial Differential Equations such as the Heat equation.

% \begin{figure}
% 	\centering
% 	\includegraphics[width=.7\columnwidth]{figures/Gauss.pdf}
% 	\caption{Dependency graph of the Gauss-Seidel Method}
% 	\label{fig:gauss}
% \end{figure}

The matrix containing the linear equation system is split into a two-dimensional grid.
Each block is computed separately but depends on the upper and left blocks, creating a pattern displayed in Figure \ref{fig:gauss-cross}.
The computation is repeated for each iteration.
Solid arrows in the Figure denote data dependencies inside an iteration, and thus tasks have to be executed from lighter to darker.

Note that due to the nature of the dependencies, when the iteration starts there is only one task to execute:
the top left task. After the first task ends, two tasks can be executed concurrently, and parallelism
grows in a wave-front pattern.
In this case, if we split the matrix into more blocks, decreasing granularity, we increase the available parallelism
without compromising the accuracy of the final result.
Additionally, note that once a block has been used as input for its neighbors, we can start computing the next iteration
right away and increase the available parallelism by having tasks from more than one iteration in flight.

Moreover, task instances in iteration $i+1$ have dependencies with task instances in the previous iteration $i$,
as shown in Figure \ref{fig:gauss-cross}. For the sake of clarity, only dependencies from block $A^k_i$, denoting
the task instance of block $k$ on iteration $i$, to block $A_{i+1}^k$ are shown using dashed arrows.
However, all other blocks also have dependencies following the same pattern.

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/Gauss-Multiplev2.pdf}
	\caption{Cross-iteration dependencies in the Gauss-Seidel method. $A_i^k$ represents the instance of task $A$ for block $k$ and iteration $i$.}
	\label{fig:gauss-cross}
\end{figure}

When we express this application in a data-flow programming model, must choose a suitable task granularity (the matrix's block size).
This choice is based on the knowledge that performance is related to task granularity, as shown in Figure \ref{fig:granularity}.
Whenever task granularity is higher than $g_1$, there are very few task instances, and they are very coarse.
This leads to the application having little parallelism, as shown in the example trace in Figure \ref{fig:granularity}c.
When granularity is between $g_0$ and $g_1$, there is a good balance between task creation overheads and parallelism, allowing to fill all the cores
as shown in Figure \ref{fig:granularity}b.
Finally, if we choose a granularity smaller than $g_0$, task instances cannot be created fast enough to feed all cores with work, leading to the performance
degradation showcased in Figure \ref{fig:granularity}a.

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figures/Granularity.pdf}
	\caption{Plot of performance versus granularity, related to typical execution traces of each scenario}
	\label{fig:granularity}
\end{figure}

In the case of the heat equation, we can measure performance versus granularity and obtain the plot
in Figure \ref{fig:granularity-heat}. Here, we can see there is an optimal granularity, and several
good performing granularities between the $g_0$ and $g_1$ points.
However, when we have a granularity smaller than $g_0$, our performance drops sharply.

\begin{figure}
	\centering
	\includegraphics[width=.9\columnwidth]{figures/TraceRealHeat.pdf}
	\caption{Granularity vs normalized performance for the heat equation on an OpenMP Tasks version}
	\label{fig:granularity-heat}
\end{figure}

Moreover, when we perform strong scaling on an application, as we increase the number of cores,
$g_1$ in Figure~\ref{fig:granularity} becomes smaller and moves to the left.
Eventually, as we keep strong scaling, $g_1$ may move past $g_0$, limiting the performance of our application.
This is one of the reasons there is a strong focus on reducing task creation and scheduling costs.

In the specific case of the heat equation and other iterative applications, code often loops for every iteration,
creating the same tasks $N$ times, where $N$ is the number of iterations.
Listing \ref{lst:heat} shows the relevant code for task creation in our example Gauss-Seidel application.
Note that instances of the same tasks with the same parameters and dependencies are created for each outer loop iteration.

\begin{lstlisting}[language=C, label=lst:heat, caption=Task creation code in a sample Gauss-Seidel Heat Equation application,float]
for (int timestep = 0; timestep < N; ++timestep) {
	for (int R = 1; R < numRowBlocks - 1; ++R) {
		for (int C = 1; C < numColumnBlocks - 1; ++C) {
			#pragma oss task label(block computation) \
					in(reps[R-1][C]) in(reps[R+1][C]) \
					in(reps[R][C-1]) in(reps[R][C+1]) \
					inout(reps[R][C])
			computeBlock(rows, cols, R, C, matrix);
		}
	}
}
\end{lstlisting}

Hence, if we have $K$ task instances for each iteration, the total number of task instances is $N\cdot K$.
However, if we could express with our programming model that each of the $K$ instances will be executed $N$ times,
and the overhead of re-executing a task is zero, we would reduce task creation overheads by a factor of $N$.

\subsection{OmpSs-2}

In this paper, we focus on the open-source task-based OmpSs-2 programming model \cite{bsc2020ompss2}.
Like OpenMP, users annotate serial application code with \texttt{\#pragma} annotations to generate
concurrent programs.
However, OmpSs-2 has several extensions to its data-flow model,
which are intended to minimize the need for global synchronization primitives such as the \texttt{taskwait} clause.
Nevertheless, we will discuss how our proposals can be applied to OpenMP.

